From Hours to Seconds: Towards 100x Faster Quantitative Phase Imaging via Differentiable Microscopy

With applications ranging from metabolomics to histopathology, quantitative phase microscopy (QPM) is a powerful label-free imaging modality. Despite significant advances in fast multiplexed imaging sensors and deep-learning-based inverse solvers, the throughput of QPM is currently limited by the speed of electronic hardware. Complementarily, to improve throughput further, here we propose to acquire images in a compressed form such that more information can be transferred beyond the existing electronic hardware bottleneck. To this end, we present a learnable optical compression-decompression framework that learns content-specific features. The proposed differentiable quantitative phase microscopy ($\partial \mu$) first uses learnable optical feature extractors as image compressors. The intensity representation produced by these networks is then captured by the imaging sensor. Finally, a reconstruction network running on electronic hardware decompresses the QPM images. In numerical experiments, the proposed system achieves compression of $\times$ 64 while maintaining the SSIM of $\sim 0.90$ and PSNR of $\sim 30$ dB on cells. The results demonstrated by our experiments open up a new pathway for achieving end-to-end optimized (i.e., optics and electronic) compact QPM systems that may provide unprecedented throughput improvements.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
